Agentic Ensemble with Vision-Language Models for Visual Anomaly Detection

Visual anomaly detection aims to detect abnormal objects, while anomaly samples are often scarce during model training. Assembling multiple pretrained detectors can help by leveraging their transferable image scores and anomaly maps. However, most existing ensemble methods apply fixed fusion rules over saved predictions which struggle when pretrained detectors clearly disagree due to different training objectives, priors, and visual representations. To this end, we design AnomalyAgent, a post-training fusion framework for accurate visual anomaly detection. AnomalyAgent aligns heterogeneous scores and maps, summarizes score- and region-level disagreement, and treats fusion as a finite action-selection problem. It implements two types of actions: 1) score actions that determine how to fuse image-level detector confidence via consensus, robust aggregation, detector weighting, or score-map consistency; 2) map actions that fuse dense anomaly responses via consensus, detector weighting, geometric aggregation, or disagreement correction. A constrained vision-language model (VLM) is introduced to inspect high-conflict samples and select valid score action and map action to produce the final prediction. We evaluate AnomalyAgent on MVTec AD and VisA as primary benchmarks, together with seven additional public anomaly benchmarks and Real-IAD for large-scale score-level evaluation. Across these benchmarks, AnomalyAgent consistently improves over equal-weight fusion and achieves the best mean image AUROC and pixel AP among the compared fusion methods on MVTec AD and VisA, while demonstrating robust transfer across additional anomaly domains.

==> sec/B_prompt.tex <==
\begin{figure*}[t]
\centering
\begin{tcolorbox}[
    width=0.96\textwidth,
    colback=gray!4,
    colframe=gray!45,
    boxrule=0.5pt,
    arc=1pt,
    left=5pt,
    right=5pt,
    top=4pt,
    bottom=4pt
]
\footnotesize
\ttfamily

You are an online VLM agent for visual anomaly ensemble fusion.

\vspace{2pt}
The attached panel contains the original image, detector anomaly maps,
the equal-weight reference, detector disagreement, and candidate-region
overlays.

\vspace{4pt}
\textbf{Task.}
Select one IMAGE fusion primitive and one PIXEL fusion primitive from the
provided candidates.
Do not generate a new anomaly score or mask.

\vspace{4pt}
\textbf{Decision rules.}
\begin{itemize}
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
    \item Prefer conservative primitives when detector evidence is weak.
    \item Use equal-weight fusion when adaptive responses are unsupported.
    \item Use disagreement suppression for diffuse or isolated responses.
    \item Use weighted or geometric fusion when one detector, or detector consensus, is clearly more reliable.
    \item Return only primitive names from the provided action sets.
\end{itemize}

\textbf{Output format.}
\begin{lstlisting}[basicstyle=\ttfamily\footnotesize,
                   columns=fullflexible,
                   frame=none,
                   aboveskip=2pt,
                   belowskip=0pt]
{
  "image_choice": "<image primitive>",
  "pixel_choice": "<pixel primitive>",
  "summary": "<short reason>"
}
\end{lstlisting}

\end{tcolorbox}
\caption{Prompt template for the constrained VLM fusion policy.
Dataset-specific statistics and valid action identifiers are inserted programmatically.}
\label{fig:agent-prompt-template}
\end{figure*}
